GypSum: Learning Hybrid Representations for Code Summarization

Code summarization with deep learning has been widely studied in recent years. Current deep learning models for code summarization generally follow the principle in neural machine translation and adopt the encoder-decoder framework, where the encoder learns the semantic representations from source code and the decoder transforms the learnt representations into human-readable text that describes the functionality of code snippets. Despite they achieve the new state-of-the-art performance, we notice that current models often either generate less fluent summaries, or fail to capture the core functionality, since they usually focus on a single type of code representations. As such we propose GypSum, a new deep learning model that learns hybrid representations using graph attention neural networks and a pre-trained programming and natural language model. We introduce particular edges related to the control flow of a code snippet into the abstract syntax tree for graph construction, and design two encoders to learn from the graph and the token sequence of source code, respectively. We modify the encoder-decoder sublayer in the Transformer's decoder to fuse the representations and propose a dual-copy mechanism to facilitate summary generation. Experimental results demonstrate the superior performance of GypSum over existing code summarization models.

==> sections/data_distrubtion.tex <==
\iffalse
\begin{figure}[!htb]
  \centering
    \subfigure[Code length of java dataset]{\includegraphics[width=0.22\textwidth]{figures/java_code_length.png}} 
	\subfigure[Comment length of java dataset]{\includegraphics[width=0.22\textwidth]{figures/java_comment_length.png}} \\
    \subfigure[Code length of python dataset]{\includegraphics[width=0.22\textwidth]{figures/python_code_length.png}} 
	\subfigure[Comment length of python dataset]{\includegraphics[width=0.22\textwidth]{figures/python_comment_length.png}} \\
  \caption{Length distribution of test set}
	\label{fig:data_distribution}
	\vspace{0.06in}
\end{figure}


\begin{figure}[!htb]
  \centering
    \subfigure[Overlap ratio of java dataset]{\includegraphics[width=0.22\textwidth]{figures/数据重合比例直方图_java.png}} 
	\subfigure[Overlap ratio of python dataset]{\includegraphics[width=0.22\textwidth]{figures/数据重合比例直方图_py.png}} \\
  \caption{Overlap ratio between test set and training set. The method that we use is the similarity matching algorithm. The x-axis indicates the degree of overlap and the y-axis shows how many samples there are in the test set.}
	\label{fig:overlap_ratio}
	\vspace{0.06in}
\end{figure}
\fi
